Improvisation through Physical Understanding: Using Novel Objects as Tools with Visual Foresight

Machine learning techniques have enabled robots to learn narrow, yet complex tasks and also perform broad, yet simple skills with a wide variety of objects. However, learning a model that can both perform complex tasks and generalize to previously unseen objects and goals remains a significant challenge. We study this challenge in the context of "improvisational" tool use: a robot is presented with novel objects and a user-specified goal (e.g., sweep some clutter into the dustpan), and must figure out, using only raw image observations, how to accomplish the goal using the available objects as tools. We approach this problem by training a model with both a visual and physical understanding of multi-object interactions, and develop a sampling-based optimizer that can leverage these interactions to accomplish tasks. We do so by combining diverse demonstration data with self-supervised interaction data, aiming to leverage the interaction data to build generalizable models and the demonstration data to guide the model-based RL planner to solve complex tasks. Our experiments show that our approach can solve a variety of complex tool use tasks from raw pixel inputs, outperforming both imitation learning and self-supervised learning individually. Furthermore, we show that the robot can perceive and use novel objects as tools, including objects that are not conventional tools, while also choosing dynamically to use or not use tools depending on whether or not they are required.

==> preliminaries.tex <==
\section{Preliminaries} 

\subsection{Visual Foresight}

The method proposed here is built upon visual foresight \cite{ebert2018visual} a planning algorithm that leverages a visual-prediction model trained on autonomously collected data. The visual foresight algorithm consists of three phases: unsupervised data collection, predictive model training, and planning-based control via the model at test-time.


\noindent \textbf{Model training}: We train a video prediction model on the collected data. The model takes as input an image of the current time-step and a sequence of actions, and generates the corresponding sequence of future frames. This model is described in Section \ref{sec:model}.

\noindent \textbf{Planning cost function}:A goal can be provided by the user through clicking on an object and a desired goal-position, a \emph{pixel-distance cost-function} evaluates how far the designated pixel is from the goal pixels. Given a distribution over pixel positions $P_0$, our model predicts distributions over its positions $P_t$ at time $t \in \{ 1, \dots, T \}$. One way of defining the cost per time-step $c_t$ is by using the expected Euclidean distance to the goal point $d_g$, which is straight-forward to calculate from $P_t$ and $g$, as follows:
 \begin{align}
c = \sum_{t = 1, \dots, T} c_t =  \sum_{t = 1, \dots, T} \mathbb{E}_{\hat{d}_{t} \sim P_{t}} \left[\|\hat{d}_{t} - d_{g}\|_2\right] 
 \label{eq:cost}
 \end{align}
The per time-step costs $c_t$ are summed together giving the overall planing objective $c$. For multi-objective tasks with multiple designated pixels $d^{(i)}$ the costs are summed to together, and optionally weighted according to a scheme discussed in \autoref{subsec:reg_cost}.  



\subsection{Learning from Demonstrations}

We use demonstrations to train a sampling distribution, from which we sample at test time to warm-start the action optimization in the model-predictive controller. This allows has to sample complex, long-horizon action sequences, that would be extremely unlikely to sample from simple distributions such as a multi-variate Gaussian. 


